Agentic Very Much! Adoption of Coding Agent in New GitHub Projects

In previous work, we investigated the adoption of coding agents in GitHub projects, finding that it was very significant. This study follows this line of work, but analyses new projects, that were created after the previous study. In this new sample, we find that the adoption of coding agents is more than twice as high. We also find that the adoption is significantly more intensive, as the proportion of AI-assisted commits is sensibly higher, despite strong signs that we do not detect all of it.

==> rq2-All/commit_effect_sizes.tex <==
% Chi-Squared Test Results

\begin{table}[ht]
\centering
\caption{Chi-squared goodness-of-fit tests}
\label{tab:chi2_results}
\begin{tabular}{lrrrl}
\toprule
\textbf{Category} & \textbf{Chi-squared} & \textbf{p-value} & \textbf{Effect Size} & \textbf{Interpretation} \\
\midrule
All Files & 9.2704 & 0.054685 & 0.4217 & Medium \\
All Files with commits & 39.5184 & 0.000000 & inf & Large \\
File level & 40.0391 & 0.000000 & inf & Large \\
Files ignored only & 40.0173 & 0.000000 & inf & Large \\
Commits only & 45.9053 & 0.000000 & inf & Large \\
\bottomrule
\end{tabular}
\end{table}


==> rq2-All/file_effect_sizes.tex <==
% Chi-Squared Test Results

\begin{table}[ht]
\centering
\caption{Chi-squared goodness-of-fit tests}
\label{tab:chi2_results}
\begin{tabular}{lrrrl}
\toprule
\textbf{Metric} & \textbf{Chi-squared} & \textbf{p-value} & \textbf{Effect Size} & \textbf{Interpretation} \\
\midrule
Code Lines & 1292.2647 & 0.000000 & 0.2844 & Small \\
Contributors & 703.0190 & 0.000000 & 0.1747 & Small \\
Commits & 1177.3757 & 0.000000 & 0.2256 & Small \\
Total Issues & 1384.3591 & 0.000000 & 0.2342 & Small \\
Total Pull Requests & 3313.4607 & 0.000000 & 0.3813 & Medium \\
Age Years & 2353.7985 & 0.000000 & 0.2923 & Small \\
\bottomrule
\end{tabular}
\end{table}


==> rq2-Very/commit_effect_sizes.tex <==
% Chi-Squared Test Results

\begin{table}[ht]
\centering
\caption{Chi-squared goodness-of-fit tests}
\label{tab:chi2_results}
\begin{tabular}{lrrrl}
\toprule
\textbf{Category} & \textbf{Chi-squared} & \textbf{p-value} & \textbf{Effect Size} & \textbf{Interpretation} \\
\midrule
All Files & 34.0945 & 0.000001 & 0.6056 & Large \\
All Files with commits & 76.8710 & 0.000000 & inf & Large \\
File level & 81.9707 & 0.000000 & inf & Large \\
Files ignored only & 55.1677 & 0.000000 & inf & Large \\
Commits only & 43.7578 & 0.000000 & inf & Large \\
\bottomrule
\end{tabular}
\end{table}


==> rq2-Very/file_effect_sizes.tex <==
% Chi-Squared Test Results

\begin{table}[ht]
\centering
\caption{Chi-squared goodness-of-fit tests}
\label{tab:chi2_results}
\begin{tabular}{lrrrl}
\toprule
\textbf{Metric} & \textbf{Chi-squared} & \textbf{p-value} & \textbf{Effect Size} & \textbf{Interpretation} \\
\midrule
Code Lines & 369.8217 & 0.000000 & 0.2569 & Small \\
Contributors & 28.1636 & 0.000088 & 0.0613 & Negligible \\
Commits & 91.1913 & 0.000000 & 0.1104 & Small \\
Total Issues & 47.9260 & 0.000000 & 0.0739 & Negligible \\
Total Pull Requests & 165.4252 & 0.000000 & 0.1465 & Small \\
Age Years & 192.9056 & 0.000000 & 0.1635 & Small \\
\bottomrule
\end{tabular}
\end{table}

